Diversified homotopic behavior of closed orbits of some R-covered Anosov flows

We produce infinitely many examples of Anosov flows in closed 3-manifolds where the set of periodic orbits is partitioned into two infinite subsets. In one subset every closed orbit is freely homotopic to infinitely other closed orbits of the flow. In the other subset every closed orbit is freely homotopic to only one other closed orbit. The examples are obtained by Dehn surgery on geodesic flows. The manifolds are toroidal and have Seifert fibered pieces and atoroidal pieces in their torus decompositions.

==> serg.tex <==
% Definitions that use @ : 
\catcode`\@=11

% page heading on even pages gives chapter, but on same side of page
% as for odd pages. 


\newcommand{\zz}{\mbox{${\bf Z} \oplus {\bf Z}$}}
\newcommand{\pa}{\mbox{$<_{\alpha}$}}
\newcommand{\mmp}{\mbox{$[-1,1]$}}
\newcommand{\of}{\mbox{$\overline f$}}
\newcommand{\rr}{\mbox{${\cal R}$}}
\newcommand{\cd}{\mbox{${\cal D}$}}
\newcommand{\cp}{\mbox{${\cal P}$}}
\newcommand{\ct}{\mbox{${\cal T}$}}
\newcommand{\pb}{\mbox{$<_{\beta}$}}
\newcommand{\pu}{\mbox{$<_u$}}
\newcommand{\poa}{\mbox{$>_{\alpha}$}}
\newcommand{\pou}{\mbox{$>_u$}}
\newcommand{\oh}{\mbox{$\overline h$}}
\newcommand{\og}{\mbox{$\overline g$}}
\newcommand{\spr}{\mbox{${\bf S}^2 \times {\bf S}^1$}}
\newcommand{\cs}{\mbox{${\bf S}^1$}}
\newcommand{\sss}{\mbox{${\bf S}^2$}}
\newcommand{\ch}{\mbox{$\widehat{\bf C}$}}
\newcommand{\pp}{\mbox{$\Phi_{\theta}$}}
\newcommand{\ii}{\mbox{${\cal I}$}}
\newcommand{\dd}{\mbox{${\cal D}$}}
\newcommand{\ccl}{\mbox{${\cal L}$}}
\newcommand{\kk}{\mbox{${\cal K}$}}
\newcommand{\ca}{\mbox{${\cal A}$}}
\newcommand{\is}{\mbox{${\cal I}^s$}}
\newcommand{\iu}{\mbox{${\cal I}^u$}}
\newcommand{\res}{\mbox{${\cal R}^s$}}
\newcommand{\reu}{\mbox{${\cal R}^u$}}
\newcommand{\bp}{\mbox{$B^+$}}
\newcommand{\bn}{\mbox{$B^-$}}
\newcommand{\ba}{\mbox{${\bf A}$}}
\newcommand{\aaa}{\mbox{${\cal A}$}}
\newcommand{\aap}{\mbox{${\cal A}_1$}}
\newcommand{\bb}{\mbox{${\cal B}$}}
\newcommand{\ak}{\mbox{${\cal A}_{\kappa}$}}
\newcommand{\at}{\mbox{${\cal A}_{\tau}$}}
\newcommand{\otsf}{\mbox{${\overline \tau^s_F}$}}
\newcommand{\otuf}{\mbox{${\overline \tau^u_F}$}}
\newcommand{\ots}{\mbox{${\overline \tau^s}$}}
\newcommand{\otu}{\mbox{${\overline \tau^u}$}}
\newcommand{\ap}{\mbox{${\cal A}_{\alpha}$}}
\newcommand{\ab}{\mbox{${\cal A}_{\beta}$}}
\newcommand{\ag}{\mbox{${\cal A}_g$}}
\newcommand{\lat}{\mbox{${\cal L A}_{\tau}$}}
\newcommand{\lak}{\mbox{${\cal L A}_{\kappa}$}}
\newcommand{\lal}{\mbox{${\cal L A}_{\alpha}$}}
\newcommand{\lag}{\mbox{${\cal L A}_{\gamma}$}}
\newcommand{\lab}{\mbox{${\cal L A}_{\beta}$}}
\newcommand{\la}{\mbox{${\cal L A}$}}
\newcommand{\af}{\mbox{${\cal A}_f$}}
\newcommand{\uu}{\mbox{${\cal U}$}}
\newcommand{\ro}{\mbox{${\cal R}$}}
\newcommand{\vv}{\mbox{${\cal V}$}}
\newcommand{\we}{\mbox{${\cal W}$}}
\newcommand{\re}{\mbox{${\cal R}$}}
\newcommand{\wwx}{\mbox{${\cal WX}$}}
\newcommand{\et}{\mbox{$\eta _-$}}
\newcommand{\tsv}{\mbox{$\sigma ^s_e$}}
\newcommand{\hhu}{\mbox{${\cal H} ^u$}}
\newcommand{\hhs}{\mbox{${\cal H} ^s$}}
\newcommand{\hu}{\mbox{${\cal H}(\widetilde {\cal F} ^u)$}}
\newcommand{\hs}{\mbox{${\cal H}(\widetilde {\cal F} ^s)$}}
\newcommand{\hp}{\mbox{${\cal H}$}}
\newcommand{\tup}{\mbox{$\Theta ^u_+$}}
\newcommand{\tun}{\mbox{$\Theta ^u_-$}}
\newcommand{\tsp}{\mbox{$\Theta ^s_+$}}
\newcommand{\tsn}{\mbox{$\Theta ^s_-$}}
\newcommand{\vs}{\mbox{$\varphi_s$}}
\newcommand{\vu}{\mbox{$\varphi_u$}}
\newcommand{\vg}{\mbox{$\varphi_G$}}
\newcommand{\vf}{\mbox{$\varphi_F$}}
\newcommand{\vif}{\mbox{$\varphi^{\infty}_F$}}
\newcommand{\vig}{\mbox{$\varphi^{\infty}_G$}}
\newcommand{\vil}{\mbox{$\varphi^{\infty}_L$}}
\newcommand{\vi}{\mbox{$\varphi^{\infty}$}}
\newcommand{\vr}{\mbox{$\varphi _s$}}
\newcommand{\vvv}{\mbox{${\cal V}$}}
\newcommand{\hlf}{\mbox{$X^L_F$}}
\newcommand{\hfl}{\mbox{$X^F_L$}}
\newcommand{\zf}{\mbox{$\zeta_F$}}
\newcommand{\zl}{\mbox{$\zeta_L$}}
\newcommand{\pin}{\mbox{$\partial _{\infty}$}}
\newcommand{\cc}{\mbox{$\cal C$}}
\newcommand{\lsf}{\mbox{${\cal L}^s_F$}}
\newcommand{\luf}{\mbox{${\cal L}^u_F$}}
\newcommand{\oo}{\mbox{$\cal O$}}
\newcommand{\oos}{\mbox{${\cal O}^s$}}
\newcommand{\oou}{\mbox{${\cal O}^u$}}
\newcommand{\ooo}{\mbox{$\cal J$}}
\newcommand{\uo}{\mbox{${\cal J}^u$}}
\newcommand{\so}{\mbox{${\cal J}^s$}}
\newcommand{\ou}{\mbox{${\cal J}^u_+$}}
\newcommand{\rrr}{\mbox{$\times {\bf R}$}}
\newcommand{\rrrr}{\mbox{${\bf R}$}}
\newcommand{\rp}{\mbox{$[0,+\infty)$}}
\newcommand{\pn}{\mbox{$\partial N$}}
\newcommand{\mi}{\mbox{$\widetilde M$}}
\newcommand{\wl}{\mbox{$\widetilde \lambda$}}
\newcommand{\ls}{\mbox{$\Lambda^s$}}
\newcommand{\lu}{\mbox{$\Lambda^u$}}
\newcommand{\wgs}{\mbox{$\widetilde \Lambda^s$}}
\newcommand{\wls}{\mbox{$\widetilde \Lambda^s$}}
\newcommand{\wlu}{\mbox{$\widetilde \Lambda^u$}}
\newcommand{\wcl}{\mbox{$\widetilde {\cal L}$}}
\newcommand{\wlsf}{\mbox{$\widetilde \Lambda^s_F$}}
\newcommand{\wluf}{\mbox{$\widetilde \Lambda^u_F$}}
\newcommand{\wlse}{\mbox{$\widetilde \Lambda^s_E$}}
\newcommand{\wlsg}{\mbox{$\widetilde \Lambda^s_G$}}
\newcommand{\wlsfi}{\mbox{$\widetilde \Lambda^s_{F_i}$}}
\newcommand{\wlsl}{\mbox{$\widetilde \Lambda^s_L$}}
\newcommand{\ww}{\mbox{$\widetilde W$}}
\newcommand{\wws}{\mbox{$\widetilde W^s$}}
\newcommand{\ti}{\mbox{$\partial \widetilde T$}}
\newcommand{\ttt}{\mbox{$\widetilde T$}}
\newcommand{\ppn}{\mbox{$\partial _+ N$}}
\newcommand{\lll}{\mbox{$l _{\epsilon}$}}
\newcommand{\iT}{\mbox{$i _{\widetilde T}$}}
\newcommand{\wwp}{\mbox{$\widetilde \Phi$}}
\newcommand{\wwr}{\mbox{$\widetilde \Phi_{\rrrr}$}}
\newcommand{\w}{\mbox{$\widetilde {\partial _+ C}$}}
\newcommand{\pw}{\mbox{$\varphi _{\widetilde T}$}}
\newcommand{\lmun}{\mbox{$\Gamma ^s \cup \Gamma ^u$}}
\newcommand{\gc}{\mbox{${\cal G}$}}
\newcommand{\gsgg}{\mbox{${\cal G}^s_*$}}
\newcommand{\gl}{\mbox{${\cal G}$}}
\newcommand{\gugg}{\mbox{${\cal G}^u_*$}}
\newcommand{\gsg}{\mbox{${\cal G}^s$}}
\newcommand{\gug}{\mbox{${\cal G}^u$}}
\newcommand{\ga}{\mbox{$\Gamma$}}
\newcommand{\gs}{\mbox{$\Gamma ^s$}}
\newcommand{\gu}{\mbox{$\Gamma ^u$}}
\newcommand{\ggs}{\mbox{${\cal F}^s_T$}}
\newcommand{\ggu}{\mbox{${\cal F}^u_T$}}
\newcommand{\gsr}{\mbox{$\Gamma ^s \times {\bf R}$}}
\newcommand{\gur}{\mbox{$\Gamma ^u \times {\bf R}$}}
\newcommand{\se}{\mbox{$S _{\epsilon}$}}
\newcommand{\gus}{\mbox{$\Gamma ^u \downarrow S_{\epsilon}$}}
\newcommand{\vt}{\mbox{$\overline \varphi _{\widetilde T}$}}
%\newcommand{\vvvv}{\mbox{$\varphi _{\widetilde T}$}}
\newcommand{\hh}{\mbox{${\bf H}^2$}}
\newcommand{\hhh}{\mbox{${\bf H}^3$}}
\newcommand{\lmS}{\mbox{$\Gamma ^s \downarrow S$}}
\newcommand{\lmU}{\mbox{$\Gamma ^u \downarrow S$}}
\newcommand{\lms}{\mbox{$\Gamma ^s \downarrow S_{\epsilon}$}}
\newcommand{\lmu}{\mbox{$\Gamma ^u \downarrow S_{\epsilon}$}}
\newcommand{\wall}{\mbox{$L \times \R$}}
\newcommand{\wa}{\mbox{$\widetilde {\alpha}$}}
\newcommand{\wb}{\mbox{$\widetilde {\beta}$}}
\newcommand{\wdd}{\mbox{$\widetilde {\delta}$}}
\newcommand{\lap}{\mbox{$\Gamma ^s \cup \Gamma ^u \cup Q$}}
\newcommand{\tz}{\mbox{$\widetilde T \times \{ 0 \}$}}
\newcommand{\es}{\mbox{${\cal E}^s_F$}}
\newcommand{\eu}{\mbox{${\cal E}^u_F$}}
\newcommand{\wt}{\mbox{$\widetilde T$}}
\newcommand{\wss}{\mbox{$\widetilde S$}}
\newcommand{\rs}{\mbox{$\widetilde \rho(\widetilde S)$}}
\newcommand{\trs}{\mbox{$\Theta(\widetilde \rho(\widetilde S))$}}
\newcommand{\wn}{\mbox{$\widetilde N$}}
\newcommand{\si}{\mbox{$S^2_{\infty}$}}
\newcommand{\su}{\mbox{$S^1_{\infty}$}}
%\newcommand{\sss}{\mbox{$S^s_{\infty}$}}
\newcommand{\sus}{\mbox{$S^u_{\infty}$}}
\newcommand{\s}{\mbox{$S ^1$}}
\newcommand{\fol}{\mbox{$\cal F$}}
\newcommand{\gal}{\mbox{$\cal G$}}
\newcommand{\gp}{\mbox{$\cal G_+$}}
\newcommand{\gm}{\mbox{$\cal G_-$}}
\newcommand{\gn}{\mbox{$\widetilde {\cal G}$}}
\newcommand{\gmn}{\mbox{$\widetilde {\cal G}_-$}}
\newcommand{\gpn}{\mbox{$\widetilde {\cal G}_+$}}
\newcommand{\fn}{\mbox{$\widetilde {\cal F}$}}
\newcommand{\als}{\mbox{${\cal L} ^s$}}
\newcommand{\lss}{\mbox{${\cal L}^s_*$}}
\newcommand{\alu}{\mbox{${\cal L} ^u$}}
\newcommand{\lsd}{\mbox{${\cal L} ^s_d$}}
\newcommand{\lns}{\mbox{$\widetilde {\cal L} ^s$}}
\newcommand{\lnu}{\mbox{$\widetilde {\cal L} ^u$}}
\newcommand{\fs}{\mbox{${\cal F} ^s$}}
\newcommand{\fu}{\mbox{${\cal F} ^u$}}
\newcommand{\fss}{\mbox{${\cal F} ^{ss}$}}
\newcommand{\fuu}{\mbox{${\cal F} ^{uu}$}}
\newcommand{\fuo}{\mbox{${\cal F} ^{uu}_0$}}
\newcommand{\fnss}{\mbox{$\widetilde {\cal F} ^{ss}$}}
\newcommand{\fnuu}{\mbox{$\widetilde {\cal F} ^{uu}$}}
\newcommand{\fns}{\mbox{${\widetilde {\cal F}}^s $}}
\newcommand{\fnso}{\mbox{${\widetilde {\cal F}}^s_{\cal O} $}}
\newcommand{\fnuo}{\mbox{${\widetilde {\cal F}}^u_{\cal O} $}}
\newcommand{\fnsf}{\mbox{${\widetilde {\cal F}}^s_F $}}
\newcommand{\fnsg}{\mbox{${\widetilde {\cal F}}^s_G $}}
\newcommand{\fnuf}{\mbox{${\widetilde {\cal F}}^u_F $}}
\newcommand{\fnu}{\mbox{${\widetilde {\cal F}}^u $}}
\newcommand{\wv}{\mbox{${\overline {\varphi}}$}}
\newcommand{\oxi}{\mbox{${\overline {\xi}}$}}
\newcommand{\wvv}{\mbox{${\varphi}$}}
\newcommand{\fsS}{\mbox{${\cal F} ^s_S$}}
\newcommand{\fsG}{\mbox{${\cal F} ^s_G$}}
\newcommand{\fsE}{\mbox{${\cal F} ^s_E$}}
\newcommand{\fuG}{\mbox{${\cal F} ^u_G$}}
\newcommand{\fuS}{\mbox{${\cal F} ^u_S$}}
\newcommand{\fsT}{\mbox{${\cal F} ^s_T$}}
\newcommand{\fuT}{\mbox{${\cal F} ^u_T$}}
\newcommand{\fSS}{\mbox{$\widetilde{\cal F} ^s_{\cal S}$}}
\newcommand{\fUS}{\mbox{$\widetilde{\cal F} ^u_{\cal S}$}}
\newcommand{\fnuS}{\mbox{$\widetilde {{\cal F}}^u_S $}}
\newcommand{\fnsS}{\mbox{$\widetilde {{\cal F}}^s_S $}}
\newcommand{\ws}{\mbox{$\widetilde  W^s$}}
\newcommand{\wu}{\mbox{$\widetilde  W^u$}}
\newcommand{\hnt}{homotopically non trivial}
\newcommand{\up}{\mbox{${\cal U} _+$}}
\newcommand{\un}{\mbox{${\cal U} _-$}}
\newcommand{\Dp}{\mbox{$\Delta ^+$}}
\newcommand{\Dn}{\mbox{$\Delta ^-$}}
\newcommand{\fg}{\mbox{$\phi _g$}}
\newcommand{\h}{\mbox{$\bf H$}}

 

\def\@evenhead{\rm \leftmark \hfil \thepage}%        Left heading.
\def\chaptermark#1{\markboth {\sc {\ifnum \c@secnumdepth >\m@ne
      \@chapapp\ \thechapter. \ \fi #1}}{}}%

\catcode`\@=12


